A Mixed-Methods Evaluation of LLM-Based Chatbots for Menopause

The integration of Large Language Models (LLMs) into healthcare settings has gained significant attention, particularly for question-answering tasks. Given the high-stakes nature of healthcare, it is essential to ensure that LLM-generated content is accurate and reliable to prevent adverse outcomes. However, the development of robust evaluation metrics and methodologies remains a matter of much debate. We examine the performance of publicly available LLM-based chatbots for menopause-related queries, using a mixed-methods approach to evaluate safety, consensus, objectivity, reproducibility, and explainability. Our findings highlight the promise and limitations of traditional evaluation metrics for sensitive health topics. We propose the need for customized and ethically grounded evaluation frameworks to assess LLMs to advance safe and effective use in healthcare.

==> oldabstract.tex <==
The integration of Large Language Models (LLMs) into healthcare settings has gained significant attention, particularly for supporting question-answering tasks for both clinicians and patients. 
Given the high-stakes nature of healthcare, it is essential to ensure that LLM-generated content is accurate and reliable to prevent adverse outcomes. However, the development of robust metrics and methodologies for evaluating these systems remains a matter of much debate. 
This paper examines the performance of publicly available LLM-based chatbots in addressing menopause-related queries, using a mixed-methods approach to evaluate safety, consensus, objectivity, reproducibility, and explainability. 
Our findings highlight both the promise of LLMs in providing menopause-related information and the limitations of traditional evaluation metrics for sensitive health topics. 
We propose the need for customized evaluation frameworks to assess LLM chatbots to advance their safe and effective use, especially in patient-facing settings.
